Causality for VARMA processes with instantaneous effects: The global Markov property, faithfulness and instrumental variables

Causal reasoning has gained great attention over the last half century as it allows (or at least intends) to answer questions which go above those within the capabilities of classical inferential statistics using just observational data. So far, causal research has been focused mostly on the i.i.d. setting. However, many are the situations where there exists a non-trivial dependence structure between sequential observations. Motivated by this fact, the main purpose of this work is to study causal properties of time series under the structural assumption of a VARMA model with instantaneous effects. First, the global Markov property is studied, building on existing work for VAR processes without instantaneous effects. Infinite graphs which represent the dependencies of the process are defined so that separation statements translate to conditional independencies in the stationary distribution of the process. Second, faithfulness is examined as a counterpart of this Markov property. Conditions are given so that the stationary distribution of the process is almost surely faithful to said infinite graphs. In addition, an instrumental variable regression framework is developed for VARMA models with instantaneous effects. This allows to identify and consistently estimate total causal effects.

==> Sections/VarmaWithout.tex <==
\section{The global Markov property for VARMA processes without instantaneous effects}\label{sec:VarmaWithout}
\begin{definition}[VARMA process without instantaneous effects \cite{hamilton2020time}]\label{def:VARMAWithout}
    We say that a (weakly stationary) time series $S$ follows a VARMA($p,q$) process without instantaneous effects if there exist $p,q\in\mathbb{N}$ and coefficient matrices $A_1,\ldots,A_p,B_1,,\ldots,B_q\in\mathbb{R}^{d\times d}$ such that for all $t\in\mathbb{Z}$: $$S_t=A_1S_{t-1}+\ldots +A_pS_{t-p}+\varepsilon_t+B_1\varepsilon_{t-1}+\ldots B_q\varepsilon_{t-q},$$ where $A_1,\ldots,A_p$ are such that $\det (I_d\lambda^p-A_1\lambda^{p-1}-\ldots -A_p)=0$ implies $|\lambda|<1$, and  $\varepsilon_t\overset{\text{i.i.d.}}{\sim}\mathcal{N}(0,\Gamma)$, with $\Gamma$ a diagonal matrix. We define the full-time graph of this process $\mathcal{G}_{full}$ as an infinite directed graph over nodes $\{S_t^i,\varepsilon_t^i\colon i\in\{1,\ldots,d\},\ t\in\mathbb{Z}\}$ such that:
    \begin{itemize}
        \item For $t\in\mathbb{Z}$ and $k\in\{1,\ldots,p\}$ there is an edge from $S_{t-k}^j$ to $S_t^i$ if $(A_k)_{i,j}\neq 0$,
        \item for $t\in\mathbb{Z}$ and $l\in\{1,\ldots,q\}$ there is an edge from $\varepsilon_{t-l}^j$ to $S_t^i$ if $(B_l)_{i,j}\neq 0$,
        \item for $t\in\mathbb{Z}$ and $i\in\{1,\ldots,d\}$ there is an edge from $\varepsilon_{t}^i$ to $S_t^i$.
    \end{itemize}
     We assume this graph to be acyclic. 
\end{definition}
% \begin{remark}
%     Note how in the case $q=0$ we have a VAR($p$) process as in Definition \ref{def:VARWithout}. In that case, the nodes representing the innovations and the edges $\varepsilon_{t}^i\to S_t^i$ are omitted as there are the only nodes related to each innovation term, and hence do not affect $d$-separation statements in the full-time DAG.
% \end{remark}
The condition imposed in Definition \ref{def:VARMAWithout} on the coefficient matrices $A_1,\ldots,A_p$ guarantees the VARMA process admits an MA($\infty$) representation, as detailed in \cite{hamilton2020time}. However, a complication arises when studying which innovations enter the MA($\infty$) representation of each component of the process. For a VAR($p$) process (which is formally a VARMA($p,0$) process)  as those studied in \cite{thams2022identifying}, it is clear by iterating the structural equations that the innovations which enter the MA($\infty$) of a certain components of the process are those associated with the nodes in its ancestral set with respect to the full-time DAG.  While in a VARMA process we can still make a one-to-one identification between components of the process at each time point and each innovation, due to the MA part of the process, it might happen that $\varepsilon_t^i$ enters the MA($\infty$) representation of a node  which does not have $S_t^i$ as an ancestor. The following proposition allows us to characterize the set of innovations taking part in the MA($\infty$) representation of a certain component of the process.
\begin{restatable}{proposition}{propMArepVarma}\label{prop:MArepVarma}
    Let $S$ be a VARMA($p,q$) process as per Definition \ref{def:VARMAWithout}, with associated full-time DAG $\mathcal{G}_{full}$. For $t\in\mathbb{Z}$ and $i\in\{1,\ldots,d\}$, the innovations which can enter the MA($\infty$) representation of $S_t^i$ are: $$\{\varepsilon_s^j\colon\varepsilon_s^j\in AN_{\mathcal{G}_{full}}(S_t^i), s\in\mathbb{Z}_{\leq t},j\in\{1,\ldots,d\}\}.$$
\end{restatable}
% \begin{proof}
%     By iterating the structural equation of the process, we can see that, for all $t\in\mathbb{Z}$: 
%     \begin{equation*}
%         \begin{split}
%         S_t&=\varepsilon_t\\&+\sum_{n=0}^\infty\left[\sum_{i_1=1}^p\dots\sum_{i_n=1}^pA_{i_1}\dots A_{i_n}\left(\sum_{l=1}^qB_l\varepsilon_{t-l-\sum_{k=1}^ni_k}+\sum_{j=1}^pA_j\varepsilon_{t-j-\sum_{k=1}^ni_k}\right)\right]
%     \end{split},
%     \end{equation*}
%     where we see that $\varepsilon_s^j$ can only enter the MA($\infty$) representation of $S_t^i$ (with $s<t$) either if $S_s^j$ is an ancestor of $S_t^i$ using the instantaneous edge $\varepsilon_s^j\to S_s^j$, or using a non-instantaneous edge ($(B_l)_{w,j}\neq 0$) to $S_{s+l}^w$ an ancestor of $S_t^i$. In both cases, $\varepsilon_s^j$ is an ancestor of $S_t^i$ in the full-time DAG $\mathcal{G}_{full}$.
% \qed\end{proof}
The problem with the full-time DAG of a VARMA process is that it has nodes representing the innovations. This is clearly sub-optimal, as the innovations are not an observed part of the process. We would then like to construct a graph  over the observed nodes which also conveys the information related to the latent nodes (the innovations). To do so we first introduce latent projections: 
\begin{definition}[Latent projection of a DAG \cite{tian2012testable}]\label{def:LatentProjection}
    Let $\mathcal{G}$ be a DAG over a finite set of nodes $V\cup L$ disjoint. The latent projection of $\mathcal{G}$ over $V$, denoted a $\mathcal{G}_V$ is an ADMG over $V$ such that, for all $v,w\in V$ there is:
    \begin{itemize}
        \item A directed edge $v\to w$ if and only if $v\to w$ exists in $\mathcal{G}$ or  there exist $m\in\mathbb{N}$, $v_1,\ldots,v_m\not\in V$, and a directed path $v\to v_1\to\cdots\to v_m\to w$ in $\mathcal{G}$, and
        \item a bi-directed edge $v\leftrightarrow w$ if and only if exist $m,n\in\mathbb{N}$, $v_1,\ldots,v_n,w_1,\ldots,w_m$, $U\not\in V$ such that there exist directed paths $U\to v_1\to\cdots\to v_n\to v$ and $U\to w_1\to\cdots\to w_m\to w$ in $\mathcal{G}$.
    \end{itemize}
\end{definition}
\begin{remark}
    All directed edges in $V$ are preserved by the latent projection operation. Therefore, the sets of parents, descendants and ancestors on nodes of $V$ in $V$ do not change in the latent projection, as these concepts involve only directed edges. 
\end{remark}
The idea of a latent projection was to find a ``simpler'' graph over $V$ which conveyed the same information as the original DAG. The following result shows that this is indeed achieved:
\begin{proposition}[Separation equivalence under latent projection \cite{richardson2023nested}]\label{prop:SeparationEquivLatentProjection}
    Let $\mathcal{G}$ a DAG over nodes $V\cup L$ disjoint and $\mathcal{G}_V$ its latent projection. Let $A,B,C\subset V$ disjoint sets of nodes. Then $A$ and $C$ are $d$-separated by $B$ in $\mathcal{G}$ if and only if they are $m$-separated by $B$ in $\mathcal{G}_V$.
\end{proposition}
Definition \ref{def:LatentProjection} does not apply directly to the full-time DAG of a VARMA process, as this DAG is infinite. Nevertheless, due to the repetitive structure of this DAG, we can consider the latent projection of a large-enough time-frame, and then iterate the structure of the resulting ADMG. We then obtain the marginalized full-time graph:
\begin{definition}[Marginalized full-time graph of a VARMA process]
    Consider a time series $S$ following a VARMA($ p, q$) process as per Definition \ref{def:VARMAWithout}, and let $\mathcal{G}_{full}$ be its full-time DAG. Its marginalized full-time graph is an infinite ADMG over the nodes $\{S_t^i\colon t\in\mathbb{Z}, i\in\{1,\ldots,d\}\}$ constructed the following way: for an arbitrary $t^*\in\mathbb{Z}$, consider the proper subgraph of $\mathcal{G}_{full}$ over nodes  $\{S_t^i,\varepsilon_t^i\colon t\in\{t^*-\max(p,q)-1,\ldots,t^*\}, i\in\{1,\ldots,d\}\}$, and then its latent projection over $\{S_t^i\colon t\in\{t^*-\max(p,q)-1,\ldots,t^*\}, i\in\{1,\ldots,d\}\}$; the marginalized full-time graph is then obtained by infinitely repeating the structure of this ADMG. We denote it by $(\mathcal{G}_{full})_S$, or simply by $\mathcal{G}_S$.
\end{definition}
\begin{remark}
    A more general definition of the marginalization of an infinite full-time DAG can be found in \cite{thams2022identifying}. While the definition comes in the context of VAR processes, it can be straightforwardly generalized to the full-time DAG of a VARMA process.
\end{remark}
\begin{example}\label{ex:VarmaWithout}
    Consider for example the 2-dimensional VARMA(1,1) process: 
    \begin{equation}\label{eq:ExampleVarmaDAG}
        \begin{cases}
            X_t=\frac{1}{2}X_{t-1}+\varepsilon_t^X+\frac{1}{4}\varepsilon_{t-1}^Y\\
            Y_t=\frac{1}{3}X_{t-1}+\frac{1}{2}Y_{t-1}+\varepsilon_t^Y
        \end{cases},
    \end{equation}
    with $\varepsilon_t\overset{\text{i.i.d.}}{\sim}\mathcal{N}(0,I_2)$. Its associated full-time DAG $\mathcal{G}_{full}$ can be seen in Figure \ref{fig:ExampleVarmaDAG}.
    \begin{figure}
        \centering
        \begin{tikzpicture}[
        main/.style={draw, circle, thick, minimum size=12mm}
        ]
        %Nodes
        % \node[squarednode]      (maintopic)                              {2};
        % \node[roundnode]        (uppercircle)       [above=of maintopic] {1};
        % \node[squarednode]      (rightsquare)       [right=of maintopic] {3};
        % \node[roundnode]        (lowercircle)       [below=of maintopic] {4};
        \node[main] (xt) {$X_t$};
        \node[main] (yt) [below = of xt] {$Y_t$};
        \node[main] (xt-1) [left =  of xt]{$X_{t-1}$};
        \node[main] (yt-1) [below = of xt-1] {$Y_{t-1}$};
        \node[main] (xt-2) [left =  of xt-1]{$X_{t-2}$};
        \node[main] (yt-2) [below = of xt-2] {$Y_{t-2}$};
        \node[main] (xt+1) [right =  of xt]{$X_{t+1}$};
        \node[main] (yt+1) [below = of xt+1] {$Y_{t+1}$};
        \node[main, draw=none] (top) [right = of xt+1] {};
        \node[main, draw=none] (bot) [below = of top] {};
        \node[main, draw=none] (pasttop) [left = of xt-2] {};
        \node[main, draw=none] (pastbot) [below = of pasttop] {};
                % innovations
        \node[main] (ext)[above = of xt] {$\varepsilon^X_t$};
        \node[main] (eyt) [below = of yt] {$\varepsilon^Y_t$};
        \node[main] (ext-1) [left =  of ext]{$\varepsilon^X_{t-1}$};
        \node[main] (eyt-1) [below = of yt-1] {$\varepsilon^Y_{t-1}$};
        \node[main] (ext-2) [left =  of ext-1]{$\varepsilon^X_{t-2}$};
        \node[main] (eyt-2) [below = of yt-2] {$\varepsilon^Y_{t-2}$};
        \node[main] (ext+1) [right =  of ext]{$\varepsilon^X_{t+1}$};
        \node[main] (eyt+1) [below = of yt+1] {$\varepsilon^Y_{t+1}$};
        % \node[main, draw=none] (etop) [right = of ext+1] {};
        % \node[main, draw=none] (ebot) [below = of bot] {};
        %\node[main, draw=none] (epasttop) [left = of ext-2] {};
        \node[main, draw=none] (epastbot) [below = of pastbot] {};
        
        %Lines
        \draw[-{Stealth[length=2.5mm]}] (xt.south) --  (yt+1.north);
        \draw[-{Stealth[length=2.5mm]}] (xt-1.east) -- node[above] {$\frac{1}{2}$} (xt.west);
        \draw[-{Stealth[length=2.5mm]}] (yt-1.east) -- node[pos=0.2, above] {$\frac{1}{2}$} (yt.west);
        \draw[-{Stealth[length=2.5mm]}] (xt-1.south) -- node[right, above] {$\frac{1}{3}$} (yt.north);
        \draw[-{Stealth[length=2.5mm]}] (xt.east) -- (xt+1.west);
        \draw[-{Stealth[length=2.5mm]}] (yt.east) -- (yt+1.west);
        \draw[-{Stealth[length=2.5mm]}] (xt-2.east) -- (xt-1.west);
        \draw[-{Stealth[length=2.5mm]}] (yt-2.east) -- (yt-1.west);
        \draw[-{Stealth[length=2.5mm]}] (xt-2.south) -- (yt-1.north);
        \draw[-{Stealth[length=2.5mm]}] (xt+1.south) --  (bot.north);
        \draw[-{Stealth[length=2.5mm]}] (xt+1.east) -- (top.west);.
        \draw[-{Stealth[length=2.5mm]}] (yt+1.east) -- (bot.west);
        \draw[-{Stealth[length=2.5mm]}] (pasttop.east) -- (xt-2.west);
        \draw[-{Stealth[length=2.5mm]}] (pastbot.east) -- (yt-2.west);
        \draw[-{Stealth[length=2.5mm]}] (pasttop.south) -- (yt-2.north);
        % \draw[-{Stealth[length=2.5mm]}] (uppercircle.south) -- (maintopic.north);
        % \draw[-{Stealth[length=2.5mm]}] (maintopic.east) -- (rightsquare.west);
        % \draw[-{Stealth[length=2.5mm]}] (rightsquare.south) .. controls +(down:7mm) and +(right:7mm) .. (lowercircle.east);
                %innovvations
        \draw[-{Stealth[length=2.5mm]}] (ext.south) --  (xt.north);
        \draw[-{Stealth[length=2.5mm]}] (ext-1.south) --  (xt-1.north);
        \draw[-{Stealth[length=2.5mm]}] (ext-2.south) --  (xt-2.north);
        \draw[-{Stealth[length=2.5mm]}] (ext+1.south) --  (xt+1.north);
        \draw[-{Stealth[length=2.5mm]}] (eyt.north) --  (yt.south);
        \draw[-{Stealth[length=2.5mm]}] (eyt-1.north) --  (yt-1.south);
        \draw[-{Stealth[length=2.5mm]}] (eyt-2.north) --  (yt-2.south);
        \draw[-{Stealth[length=2.5mm]}] (eyt+1.north) --  (yt+1.south);
        \draw[-{Stealth[length=2.5mm]}] (eyt.north) --  (xt+1.south);
        \draw[-{Stealth[length=2.5mm]}] (eyt-1.north) -- node[pos=0.3,below] {$\frac{1}{4}$}  (xt.south);
        \draw[-{Stealth[length=2.5mm]}] (eyt-2.north) --  (xt-1.south);
        \draw[-{Stealth[length=2.5mm]}] (epastbot.north) --  (xt-2.south);
        \draw[-{Stealth[length=2.5mm]}] (eyt+1.north) --  (top.south);
        
    \end{tikzpicture}
    \caption[Full-time DAG  for the process  defined in  \eqref{eq:ExampleVarmaDAG}.]{Full-time DAG of the time series  defined in Equation \eqref{eq:ExampleVarmaDAG}. The coefficients of the edges correspond with the coefficients of the process.}
  %   \caption[Geyser data: binned histogram, Silverman's and another
  % kernel]%<<-- Legend for the list of figures at the beginning of you thesis
  % {Old Faithful Geyser eruption lengths, $n=272$; binned data and two
  %   (Gaussian) kernel density estimates ($\times 10$) with $h=h^*= .3348$
  %   and $h= .1$ (dotted).}% legend displayed below the graph.
    \label{fig:ExampleVarmaDAG}
    \end{figure}
    The marginalized full-time ADMG $\mathcal{G}_S$ associated with the process defined in Equation \eqref{eq:ExampleVarmaDAG} can be found in Figure \ref{fig:ExampleVarmaADMG}. We see how this graph has both directed and bi-directed edges. We can use the ADMG in Figure \ref{fig:ExampleVarmaADMG} to exemplify the $m$-separation criterion (Definition \ref{def:mSep}), as $X_t\perp_{\mathcal{G}_{S}}Y_t|\{X_{t-1},Y_{t-1}\}$. Furthermore, Proposition \ref{prop:SeparationEquivLatentProjection} implies that $X_t\perp_{\mathcal{G}_{full}}Y_t|\{X_{t-1},Y_{t-1}\}$, what we can easily check in Figure \ref{fig:ExampleVarmaDAG}.
    \begin{figure}
        \centering
        \begin{tikzpicture}[
        main/.style={draw, circle, thick, minimum size=12mm}
        ]
        %Nodes
        % \node[squarednode]      (maintopic)                              {2};
        % \node[roundnode]        (uppercircle)       [above=of maintopic] {1};
        % \node[squarednode]      (rightsquare)       [right=of maintopic] {3};
        % \node[roundnode]        (lowercircle)       [below=of maintopic] {4};
        \node[main] (xt) {$X_t$};
        \node[main] (yt) [below = of xt] {$Y_t$};
        \node[main] (xt-1) [left =  of xt]{$X_{t-1}$};
        \node[main] (yt-1) [below = of xt-1] {$Y_{t-1}$};
        \node[main] (xt-2) [left =  of xt-1]{$X_{t-2}$};
        \node[main] (yt-2) [below = of xt-2] {$Y_{t-2}$};
        
        \node[main] (xt+1) [right =  of xt]{$X_{t+1}$};
        \node[main] (yt+1) [below = of xt+1] {$Y_{t+1}$};
        \node[main, draw=none] (top) [right = of xt+1] {};
        \node[main, draw=none] (bot) [below = of top] {};
        \node[main, draw=none] (pasttop) [left = of xt-2] {};
        \node[main, draw=none] (pastbot) [below = of pasttop] {};
        %Lines
        \draw[-{Stealth[length=2.5mm]}] (xt.south) --  (yt+1.north);
        \draw[-{Stealth[length=2.5mm]}] (xt-1.east) --  (xt.west);
        \draw[-{Stealth[length=2.5mm]}] (yt-1.east) --  (yt.west);
        \draw[-{Stealth[length=2.5mm]}] (xt-1.south) --  (yt.north);
        \draw[-{Stealth[length=2.5mm]}] (xt.east) -- (xt+1.west);
        \draw[-{Stealth[length=2.5mm]}] (yt.east) -- (yt+1.west);
        \draw[-{Stealth[length=2.5mm]}] (xt-2.east) -- (xt-1.west);
        \draw[-{Stealth[length=2.5mm]}] (yt-2.east) -- (yt-1.west);
        \draw[-{Stealth[length=2.5mm]}] (xt-2.south) -- (yt-1.north);
        \draw[-{Stealth[length=2.5mm]}] (xt+1.south) --  (bot.north);
        \draw[-{Stealth[length=2.5mm]}] (xt+1.east) -- (top.west);.
        \draw[-{Stealth[length=2.5mm]}] (yt+1.east) -- (bot.west);
        \draw[-{Stealth[length=2.5mm]}] (pasttop.east) -- (xt-2.west);
        \draw[-{Stealth[length=2.5mm]}] (pastbot.east) -- (yt-2.west);
        \draw[-{Stealth[length=2.5mm]}] (pasttop.south) -- (yt-2.north);
        \draw[{Stealth[length=2.5mm]}-{Stealth[length=2.5mm]}] (yt-1.north) --  (xt.south);
        \draw[{Stealth[length=2.5mm]}-{Stealth[length=2.5mm]}] (yt-2.north) --  (xt-1.south);
        \draw[{Stealth[length=2.5mm]}-{Stealth[length=2.5mm]}] (yt.north) --  (xt+1.south);
        \draw[{Stealth[length=2.5mm]}-{Stealth[length=2.5mm]}] (yt+1.north) --  (top.south);
        \draw[{Stealth[length=2.5mm]}-{Stealth[length=2.5mm]}] (pastbot.north) --  (xt-2.south);
        % \draw[-{Stealth[length=2.5mm]}] (uppercircle.south) -- (maintopic.north);
        % \draw[-{Stealth[length=2.5mm]}] (maintopic.east) -- (rightsquare.west);
        % \draw[-{Stealth[length=2.5mm]}] (rightsquare.south) .. controls +(down:7mm) and +(right:7mm) .. (lowercircle.east);
    \end{tikzpicture}
    \caption[Example of the marginalized full-time ADMG  for the process in \eqref{eq:ExampleVarmaDAG}.]{Marginalized full-time ADMG of the time series  defined in Equation \eqref{eq:ExampleVarmaDAG}.}
    \label{fig:ExampleVarmaADMG}
    \end{figure}
    It is relevant to note how directed edges in the marginalized graph represent dependencies coming from the AR part of the process, while bi-directed edges come from correlation due to the MA part. 
\end{example}
In Proposition  \ref{prop:MArepVarma} we characterized the innovations which can appear in the MA($\infty$) representation of a VARMA process as those considered in Definition \ref{def:VARMAWithout}. However, it would be useful to have a characterization of this set of innovations relating to the marginalized full-time ADMG, where we identify each node with the contemporaneous innovation which enters its structural equation. To that end, we have the following proposition:
\begin{restatable}{proposition}{propMArepVarmaADMG}\label{prop:MArepVarmaADMG}
    Let $S$ be a VARMA($p,q$) process as per Definition \ref{def:VARMAWithout}, with associated full-time DAG $\mathcal{G}_{full}$, and marginalized full-time ADMG $\mathcal{G}_S$. For $t\in\mathbb{Z}$ and $i\in\{1,\ldots,d\}$, the innovations which can enter the MA($\infty$) representation of $S_t^i$ are: $$\{\varepsilon_s^j\colon S_s^j\in SP_{\mathcal{G}_S}(AN_{\mathcal{G}_S}(S_t^i)), s\in\mathbb{Z}_{\leq t},j\in\{1,\ldots,d\}\}.$$
\end{restatable}
% \begin{proof}
%     Denote $(I)= \{\varepsilon_s^j\colon S_s^j\in SP_{\mathcal{G}_S}(AN_{\mathcal{G}_S}(S_t^i)), s\in\mathbb{Z}_{\leq t},j\in\{1,\ldots,d\}\}$ and $(II)=\{\varepsilon_t^i\}\cup\{\varepsilon_s^j\colon\varepsilon_s^j\in AN_{\mathcal{G}_{full}}(S_t^i), s\in\mathbb{Z}_{<t},j\in\{1,\ldots,d\}\}$. We  do not need to prove that $(I)=(II)$, but rather only $(II)\subset(I)$, as we only intent do give necessary conditions (we will not aim for sufficiency due to the possibility of multiple paths cancelling each other).   %\item $(I)\subset (II)$: Consider $\varepsilon_s^j\in (I)$. If $S_s^j\in AN_{\mathcal{G}_S}(S_t^i)$ then $S_s^j\in AN_{\mathcal{G}_{full}}(S_t^i)$, and as the edge $\varepsilon_s^i\to S_s^j$ exists in $\mathcal{G}_{full}$, we have that $\varepsilon_s^j\in AN_{\mathcal{G}_{full}}(S_t^i)$. Otherwise, there must exist a node $w\in AN_{\mathcal{G}_{S}}(S_t^i)$ such that $S_s^j\leftrightarrow w$ in $\mathcal{G}_S$. 
%     Let us show then that $(II)\subset (I)$: Clearly $\varepsilon_t^i\in (I)$. Now consider $\varepsilon_s^i\in (II)\backslash\{\varepsilon_t^i\}$. Then $\varepsilon_s^j\in AN_{\mathcal{G}_{full}}(S_t^i)$. As $\varepsilon_s^j$ only has outgoing edges into observed nodes, there exist $v_1,\ldots,v_m\in\{S_k^j\colon k\in\mathbb{Z}_{\geq s},j\in\{1,\ldots,d\}\}$ and a path $\varepsilon_s^j\to v_1\to\dots\to v_m\to S_t^i$. If $v_1=S_s^j$, then $S_s^j\in AN_{\mathcal{G}_{full}}(S_t^i)\subset SP_{\mathcal{G}_S}(AN_{\mathcal{G}_S}(S_t^i))$. Otherwise the structure $S_s^j\leftarrow\varepsilon_s^j\to v_1$ marginalizes to $S_s^j\leftrightarrow v_1$ in $\mathcal{G}_S$, meaning $S_s^j\in SP_{\mathcal{G}_S}(AN_{\mathcal{G}_S}(S_t^i))$, as we wanted to show. This concludes the proof.  \qed
% \end{proof}
When we are comparing the MA($\infty$) representations of two disjoint finite sets of nodes $A,B$ in the marginalized full-time ADMG, following Proposition \ref{prop:MArepVarmaADMG}, we would be tempted to say that these representations contain no common innovations if $SP_{\mathcal{G}_S}(AN_{\mathcal{G}_S}(A))\cap SP_{\mathcal{G}_S}(AN_{\mathcal{G}_S}(B))=\emptyset$. While this condition is sufficient, it can be slightly relaxed, as in the following corollary:
\begin{restatable}{corollary}{coroDisjointMArepVarmaWithout}\label{coro:DisjointMArepVarmaWithout}
    Consider a VARMA($p,q$) process $S$ as per Definition \ref{def:VARMAWithout}. Let $A,B$ be two finite disjoint sets of nodes of its marginalized full-time ADMG $\mathcal{G}_S$. If $AN_{\mathcal{G}_S}(A)\cap AN_{\mathcal{G}_S}(B)=\emptyset$ and there are no bi-directed edges between these two ancestral sets, then their MA($\infty$) representations have no common innovations.
\end{restatable}
% \begin{proof}
%     Assume otherwise. If $\Tilde{\varepsilon}$ appears in the MA($\infty$) representation of $A$ and $B$, due to Proposition \ref{prop:MArepVarma}, $\Tilde{\varepsilon}$ is an ancestor of $A$ and $B$ in the full-time DAG $\mathcal{G}_{full}$. This means there exist $n,m\in\mathbb{N}$ and $v_1,\ldots,v_n,w_1,\ldots,w_m\in\{S_t^i\colon t\in\mathbb{Z},j\in\{1,\ldots,d\}\}$ such that the paths $\Tilde{\varepsilon}\to v_1\to\dots\to v_n\to A$ and $\Tilde{\varepsilon}\to w_1\to\dots\to w_m\to B$ exist in $\mathcal{G}_{full}$. If $v_1=w_1$, then $A$ and $B$ have a common ancestor in $\mathcal{G}_S$. Otherwise, the structure $v_1\leftarrow\Tilde{\varepsilon}\to w_1$ in the full-time DAG marginalizes to $v_1\leftrightarrow w_1$ in $\mathcal{G}_S$, meaning there is a bi-directed edge between the two ancestral sets. \qed
% \end{proof}
At this point we have all the required tools to prove the global Markov property for VARMA processes without instantaneous effect, as presented in the following theorem:
\begin{restatable}[Global Markov property for VARMA processes]{theorem}{thmGmpVARMA} \label{thm:GmpVARMA}
    Consider $p,q\in\mathbb{N}$, and $S$ a (weakly stationary) VARMA($p,q$) process as defined in \ref{def:VARMAWithout}. Consider finite disjoint sets $A,B,C$ of nodes of the marginalized full-time ADMG $\mathcal{G}_S$.  If $A$ and $C$ are $m$-separated by $B$ in $\mathcal{G}_S$, then  $A\indep C|B$.
\end{restatable}
% \begin{proof}
%       Our proof follows the ideas of the proof of the global Markov property for VAR processes presented in \cite{thams2022identifying}, generalizing it to deal with the MA part of the process. Given a time series mixed (sub)graph $\mathcal{G}$ over nodes $V$ we define: $$ V_{[s,t]}=\{S_v^i|i \in \{1,\ldots,d\} , s\leq v\leq t, S_v^i\in V\}.$$ Consider $s_0,t_0$ the largest and smallest time points respectively such that $A\cup B\cup C\subseteq V_{[s_0,t_0]}$, and let $l\in\mathbb{N}_{>\max(p,q)}$ be such that if two nodes in $V_{[s_0,t_0]}$ are $m$-connected (with empty conditioning set) in $\mathcal{G}_S$, then there is a $m$-connecting path in $\mathcal{G}_{S,[s_0-l,t_0]}$. Note that as $l>\max(p,q)$, $\mathcal{G}_{S,[s_0-l,s_0-1]}$ contains enough information to fully describe the time dependence of the process. Now consider the set: 
%     \begin{equation*}
%         \begin{split}
%             \mathcal{A}=\{n\in\mathbb{N}| & \text{ for all directed mixed graphs } \mathcal{G}^* \text{ over nodes } V^*\text{ with time indices }\\& \quad\text{between  $s_0-l$ and $t_0$ such that all directed edges in }\mathcal{G}^* \text{ point } \\&\quad\text{``forward in time'', meaning for all }k\in\mathbb{N}\text{ and }i,j\in{1,\ldots,d}\\&\quad\text{ there is no edge }S_t^i\to S_{t-k}^j, \text{ and }\mathcal{G}^* \text{ is a subgraph of the }\\&\quad\text{ full-time  marginalized ADMG } \mathcal{G}_{S}\text{ induced by } \mathcal{G}^0= \mathcal{G}^*_{[s_0-l,s_0-1]}\\&\quad \text{ and }AN_{\mathcal{G}_{S}}(V^+)_{[s_0,t_0]}=V^+, \text{ where } V^+= V^*_{[s_0,t_0]}\\&\quad\text{ and } |V^+|=n, \\&\text{ for all VARMA($p,q$) processes with structure specified by } \mathcal{G}^0,\\&\text{ for all } A^*,B,C^*\subseteq V^* \text{ such that } V^+=A^+\cup B \cup C^+ \text{ where }\\&\quad\  A^+= A^*_{[s_0.t_0]},\ C^+= C^*_{[s_0.t_0]}  \text{ and } A^*=A^+\cup (PA_{\mathcal{G}^*}(A^+)\cap V^0)\\&\quad\   \text{ and } C^*=C^+\cup (PA_{\mathcal{G}^*}(C^+)\cap V^0),\text{ with }V^0\text{ the nodes of }\mathcal{G}^0,\\&\text{ we have: }\\&\quad\ A^*\perp_{\mathcal{G}^*}C^*|B\Rightarrow A^*\indep C^*|B      \}.
%         \end{split}
%     \end{equation*}
%     The proof first shows that $\mathcal{A}=\mathbb{N}$ suffices to prove the theorem, and secondly shows that indeed $\mathcal{A}=\mathbb{N}$ by induction on $n$. Assume then that $\mathcal{A}=\mathbb{N}$. Consider $V^0=\{S_t^i\colon s_0-l\leq t\leq s_0-1,i\in\{1,\ldots,d\}\}$, $V^+= AN_{\mathcal{G}_{S}}(A\cup B\cup C)_{[s_0.t_0]}$, $V^*= V^0\cup V^+$ and $\mathcal{G}^*$ the restriction of $\mathcal{G}_{S}$ to $V^*$. Note how $A\perp_{\mathcal{G}_{S}}C|B\Rightarrow A\perp_{\mathcal{G}^*}C|B$. However, $A,B,C$ might not satisfy the conditions required for $A^*,B,C^*$. We need to expand $A$ and $C$ appropriately: 
%     \begin{enumerate}
%         \item If $V^+\neq A\cup B \cup C$, then we expand $A$ and $C$ to disjoint sets $A^+$ and $C^+$ respectively, as per Proposition \ref{prop:ExtensionADMG}, such that $V^+=A^+\cup B\cup C^+$ and still $A^+\perp_{\mathcal{G}^*}C^+|B$.
%         \item Consider $A^*= A^+\cup (PA_{\mathcal{G}^*}(A^+)\cap V^0) $ and $C^*= C^+\cup (PA_{\mathcal{G}^*}(C^+)\cap V^0)$. Note how $A^+=A^*_{[s_0,t_0]}=A^*\cap V^0$ (idem for $C^+$) as $V^+\cap V^0=\emptyset$.  Also, $A^*\cap C^*=\emptyset$, as otherwise, given than $A^+\cap C^+=\emptyset$, there would be a common parent of $A^+$ and $C^+$ not in $B$, violating $m$-separation. 
%     \end{enumerate}
%     It also holds  that  $A^*\perp_{\mathcal{G}^*}C^*|B$. Otherwise, if there is an open path from $a\in A^*$ to $c\in C^*$ given $B$, then there is an open path from $A^+$ (either $a$ or its descendant in $A^+$) to $C^+$ (either $c$ or its descendant in $C^+$) given $B$, violating $m$-separation. Now that we are under all conditions of $\mathcal{A}$, the hypothesis $\mathcal{A}=\mathbb{N}$ implies that $A^*\indep C^*|B$, what implies $A\indep C|B$ as $A\subset A^+\subset A^*$, and idem for $C$.

%     Now it rests to show that $\mathcal{A}=\mathbb{N}$. This is done by induction on $n=|V^+|$. Recall that $V^+=A^+\cup B\cup C^+$ disjoint union.  Firstly note that $A^+=\emptyset\Rightarrow A^*=\emptyset$ (idem for $C^+$). Thus for $n=1$ and $n=2$ the only non-trivial case is $A^+=\{a\}, C^+=\{c\},B=\emptyset$. As $A^*$ and $C^*$ are $m$-separated in $\mathcal{G}^*$, they are also $m$-separated in the marginalized full-time ADMG $\mathcal{G}_S$, due to the repetitive structure of the full-time marginalized graph and the fact that $\mathcal{G}^*$ contains more that $\max(p,q)$ time steps. But this is equivalent to $A^*$ and $C^*$ being $d$-separated in the full-time DAG, and hence they have no common ancestors in $\mathcal{G}_{full}$. Thus, no innovation appears in both the ancestral sets of $A^*$ and $C^*$ in $\mathcal{G}_{full}$. This means that there are no common innovations in their MA($\infty$) representations. Due to the independence of all innovation terms, we conclude that $A^*\indep C^*$.
    
%     %As  $A^*\perp_{\mathcal{G}^*}C^*$, $A^*$ and $C^*$ have no common ancestors in $\mathcal{G}^*$, but as $\mathcal{G}^*$ contains more than $p$ time steps, the repetitive structure of $\mathcal{G}_{full}$ implies that they have no common ancestors whatsoever. By iterating the structural equations (MA($\infty$) representation)  one concludes that $A^*\indep C^*$.

%     It remains to prove that $n\in\mathcal{A}\Rightarrow n+1\in\mathcal{A}$. Consider $\mathcal{G}^*,\mathcal{G}^0,\mathcal{G}^+,A^+$, $A^*,B,C^+,C^*$ as per the definition of $\mathcal{A}$ with $|V^+|=n+1$. %The basic idea is to remove a node from $V^+$, consider the independence statements granted by the induction hypothesis, and then combine them to conclude the desired independence. 
%     Recall that topological ordering also exists in ADMGs, as this is defined with respect to directed edges only. Consider then $\lambda\in V^+$ a sink node (meaning a node without descendants) in $\mathcal{G}^*$. As $V^+=A^+\cup B\cup C^+$, there are three cases to distinguish:
%     \begin{itemize}
%         \item Assume $\lambda\in A^+$. Consider $\Delta(\lambda)=PA_{\mathcal{G}^*}(\lambda)\cup SP_{\mathcal{G}^*}(\lambda)$. Then $C^*\cap \Delta(\lambda)=\emptyset$ (as otherwise $m$-separation would be violated), what implies $PA_{\mathcal{G}_{S}}(\lambda)=PA_{\mathcal{G}^*}(\lambda)\subseteq (A^*\backslash\{\lambda\})\cup B$. Then there are coefficients $\gamma\in\mathbb{R}^{|PA_{\mathcal{G}^*}(\lambda)|}$ and $\beta\in\mathbb{R}^{dq+1}$ such that the structural equation for $\lambda$ is $\lambda=\gamma^{\top}PA_{\mathcal{G}^*}(\lambda)+\beta^{\top}\varepsilon^\lambda$, where $\varepsilon^\lambda$ is a vector of all the innovations which enter the structural equation of $\lambda$ through the MA part of the process. Now consider all variables in $(A^*\cup B\cup C^*)\backslash\Delta(\lambda)$, and iterate their structural equations over the nodes in it. $\lambda$ itself does never appear as it is a sink node. Furthermore, none of the innovations in $\varepsilon^\lambda$ appear. Indeed, and innovation can only appear when iterating these structural equations if there is (in $\mathcal{G}_{full}$) a direct edge from said innovation to an ancestor of  $(A^*\cup B\cup C^*)\backslash\Delta(\lambda)$, but if this innovation also appears in $\varepsilon^\lambda$, then there is a bi-directed edge between $\lambda$ and this ancestor, meaning this ancestor is in $\Delta(\lambda)$ and hence is not iterated over, leading to said innovation not entering the structural equation. Due to the repetitive structure of $\mathcal{G}_{full}$ and the fact that $\mathcal{G}^*$ contains more than $\max(p,q)$ time steps, we conclude that after conditioning on $\Delta(\lambda)\backslash\{\lambda\}$, no innovation in the MA($\infty$) representation of $(A^*\cup B\cup C^*)\backslash\Delta(\lambda)$ appears in $\varepsilon^\lambda$. The independence structure of the innovations then yields:
        
%         %Thanks to independence of all innovations and the fact that $\lambda$ is a sink node (it does not appear in any other structural equation), we conclude that:
%         \begin{equation}\label{eq:IndependenceInA}
%             \lambda\indep (A^*\cup B \cup C^*)\backslash\Delta(\lambda)|\Delta(\lambda)\backslash\{\lambda\},
%         \end{equation} 
%         and by the weak union property $\lambda\indep C^*|(A^*\cup B)\backslash\{\lambda\}$. If $A^*=\{\lambda\}$, then this already implies $A^*\indep C^*|B$. Otherwise, $A^*\perp_{\mathcal{G}^*}C^*|B$ implies $A^*\backslash\{\lambda\}\perp_{\mathcal{G}^*}C^*|B$, which is equivalent (by Proposition \ref{prop:SeparationADMG}) to $A^*\backslash\{\lambda\}$ being separated from $C^*$ by $B$ in $(\mathcal{G}^*)^{aug}$.  Then this separation also holds in $(\mathcal{G}^*_{V^*\backslash\{\lambda\}})^{aug}$, as this graph contains no more edges. Again by Proposition \ref{prop:SeparationADMG} this separation is equivalent to $A^*\backslash\{\lambda\}\perp_{\mathcal{G}^*_{V^*\backslash\{\lambda\}}}C^*|B$. As $|V^+\backslash\{\lambda\}|=n$, applying the induction hypothesis yields $A^*\backslash\{\lambda\} \indep C^*|B$. Combining these last two conditional independence statements by the contraction property, one concludes that $A^*\indep C^*|B$.
%         \item Assume $\lambda\in C^+$. This scenario is analogous to the $\lambda\in A^+$ case.
%         \item Assume $\lambda\in B$. The $m$-separation hypothesis is equivalent to $A^*$ and $C^*$ being separated by $B$ in $(\mathcal{G}^*)^{aug}$, what implies they are also separated by $B\backslash\{\lambda\}$ in $(\mathcal{G}^*_{V^*\backslash\{\lambda\}})^{aug}$ (as this graph contains no more edges than $(\mathcal{G}^*)^{aug}$), what is equivalent to $A^*\perp_{\mathcal{G}^*_{V^*\backslash\{\lambda\}}}C^*|B\backslash\{\lambda\}$. As $|V^+\backslash\{\lambda\}|=n$, the induction hypothesis implies $A^*\indep C^*|B\backslash\{\lambda\}$. To achieve the desired independence claim, we need a second independence statement. We consider two cases:
%         \begin{itemize}
%             \item[(a)] Assume that the following conditions hold:
%             % \begin{equation}\label{eq:ConditionsA}
%             %     \begin{cases}
%             %         PA_{\mathcal{G}^+}(\lambda)\cap A^*\neq\emptyset\\\text{ or }\\AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-q,s_1-1]})\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(A^*)_{[s_0-q,s_1-1]})\neq\emptyset
%             %     \end{cases},
%             % \end{equation}
%             % then it holds that: 
%             \begin{equation}\label{eq:ConditionsA_Varma}
%                 \begin{cases}
%                     (PA_{\mathcal{G}^+}(\lambda)\cup SP_{\mathcal{G}^+}(\lambda))\cap C^*=\emptyset,\\
%                     AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]})=\emptyset\\
%                     \qquad\text{and no bi-directed edges between these ancestral sets,}\\
%                     SP_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]})=\emptyset,\\
%                     SP_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})=\emptyset
%                 \end{cases}.
%             \end{equation}
%             Our aim is to show that the conditions given in Equation \eqref{eq:ConditionsA_Varma} imply the Independence statement $\lambda\indep C^*|A^*\cup B\backslash\{\lambda\}$. Firstly note that $PA_{\mathcal{G}^+}(\lambda)\cup SP_{\mathcal{G}^+}(\lambda)\subset A^*\cup B$. Therefore, the structural equation of $\lambda$ can be written as: $$\lambda=\gamma^{\top}\underbrace{PA_{\mathcal{G}^+}(\lambda)}_{\text{conditioned on}}+\beta^{\top}PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}+\delta^{\top}\varepsilon^\lambda,$$ where $\varepsilon^\lambda$ are the innovations which enter $\lambda$'s structural equation via its MA part, and $\gamma,\beta,\delta$ are coefficient vectors of the appropriate dimension. For the variables in $C^*$ we iterate their structural equations expect for the nodes of $B\backslash\{\lambda\}$ and $PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}$ (nodes in $A^*$ cannot appear as this would violate $m$-separation), meaning we iterate the structural equations of the nodes of $C^+$ until only nodes in $B\backslash\{\lambda\}$ and $PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}$ remain. Then essentially we can write: $$C^*=\Omega\cdot\underbrace{(B\backslash\{\lambda\})}_{\text{conditioned on}}+\Xi PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}+\Psi \varepsilon^{C^*}, $$ where $\varepsilon^{C^*}$ are all the innovation that appear in the iterated equations of $C^*$, and $\Omega,\Xi,\Psi$ are real-valued coefficient matrices of the appropriate dimensions. To achieve the desired independence statement, we need to study four pair-wise comparisons:
%             \begin{itemize}
%                 \item Consider  the MA($\infty$) representations of  $PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}$ and $PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}$. As per the second condition in Equation \eqref{eq:ConditionsA_Varma}, there is no common innovation in these two representations.
%                 \item No innovation in $\varepsilon^\lambda$ can appear in the MA($\infty$) representation of the parental set $PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}$. If this happened, there would be an innovation $\Tilde{\varepsilon}$ which has a direct edge onto $\lambda$ and an ancestor of $PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}$ in the full-time DAG $\mathcal{G}_{full}$; meaning in the full-time DAG we have $$\lambda\leftarrow\Tilde{\varepsilon}\to\bullet\to\dots\to PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}, $$ which marginalizes as: $$\lambda\leftrightarrow\bullet\to\dots\to PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]},$$ and this is a contradiction with the third condition in Equation \eqref{eq:ConditionsA_Varma}.
%                 \item $\varepsilon^\lambda$ and $\varepsilon^{C^*}$ have no common innovations. Otherwise, let $\Tilde{\varepsilon}$ be such a common innovation. Then there is a node $\Tilde{c}\in C^*$ such that $\Tilde{\varepsilon}$ enters its structural equation when iterated over nodes not in $B\backslash\{\lambda\}$ and $PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}$. As $C^*=C^+\cup PA_{\mathcal{G}^*}(C^+)_{[s_0-l,s_0-1]} $ disjoint union, there are two cases to consider:
%                 \begin{itemize}
%                     \item If $\Tilde{c}\in PA_{\mathcal{G}^*}(C^+)_{[s_0-l,s_0-1]} $, as its parents only come from the past, $\Tilde{\varepsilon}$ enters its structural equation directly, through its MA part. Then in the full-time DAG we have the structure $\lambda\leftarrow\Tilde{\varepsilon}\to\Tilde{c}$, meaning in the $\mathcal{G}^*$ there is an edge $\lambda\leftrightarrow\Tilde{c}$.  However, there is also an edge $\Tilde{c}\to C^+$, meaning $\Tilde{c}\in PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}$. This contradicts with $SP_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]})=\emptyset$.
%                     \item If $\Tilde{c}\in C^+$, then $\varepsilon$ enters its iterated structural equation either directly or by the MA part of the structural equation of a node in $PA_{\mathcal{G}^*}(\Tilde{c})_{[s_0,t_0]}$. This means that in $\mathcal{G}^*$ there is a bi-directed edge $\lambda\leftrightarrow (PA_{\mathcal{G}^*}(\Tilde{c})_{[s_0,t_0]}\cup\{\Tilde{c}\})\subseteq C^+$. This is a contradiction with $SP_{\mathcal{G}^+}(\lambda)\cap C^*=\emptyset$.
%                 \end{itemize}
%                 \item No innovation in $\varepsilon^{C^*}$ can appear in the MA($\infty$) representation of the parental set $PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}$. Consider again an innovation $\Tilde{\varepsilon}$ such that this happened. As  $\Tilde{\varepsilon}$ enters this MA($\infty$) representation, then in the full-time DAG we find the edge $\Tilde{\varepsilon}\to AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}) $. Furthermore, let again $\Tilde{c}$ be a node in $C^*$ such that $\Tilde{\varepsilon}$ enters its iterated structural equation. Again, we separate two scenarios:
%                 \begin{itemize}
%                     \item If $\Tilde{c}\in PA_{\mathcal{G}^*}(C^+)_{[s_0-l,s_0-1]} $, in the full-time DAG we find $\Tilde{\varepsilon}\to\Tilde{c}\to C^+$, which leads to the edge  $\Tilde{c}\leftrightarrow AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})$ in $\mathcal{G}^*$,  what is a contradiction with Equation \eqref{eq:ConditionsA_Varma}.
%                     \item If $\Tilde{c}\in C^+$, by the same argument as  before we have the structure $\Tilde{\varepsilon}\to (PA_{\mathcal{G}^*}(\Tilde{c})_{[s_0,t_0]}\cup\{\Tilde{c}\})$ in the full-time DAG. This leads again to a bi-directed edge $C^*\leftrightarrow AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})$ in $\mathcal{G}^*$, contradicting again the conditions in Equation \eqref{eq:ConditionsA_Varma}.
%                 \end{itemize}
%             \end{itemize}
%             Therefore, the independence structure of the innovations, together with the previous considerations imply that $\lambda\indep C^*|A^*\cup B\backslash\{\lambda\}$. Together with $A^*\indep C^*|B\backslash\{\lambda\}$, the contraction property followed by the weak-union property allow us to conclude that $C^*\indep A^*|B$.
            
%             \item[(b)] Now assume the complement of the conditions in Equation \eqref{eq:ConditionsA_Varma}:
%             \begin{equation}\label{eq:ConditionsB_Varma}
%                 \begin{cases}
%                     (PA_{\mathcal{G}^+}(\lambda)\cup SP_{\mathcal{G}^+}(\lambda))\cap C^*\neq\emptyset,\\\text{ or}\\
%                     AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]})\neq\emptyset\\
%                     \qquad\text{or there is a bi-directed edge between these ancestors,}\\
%                     \text{ or }\\
%                     SP_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]})\neq\emptyset,\\
%                     \text{ or }\\
%                     SP_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\neq\emptyset
%                 \end{cases}.
%             \end{equation}
%             Assuming any of the ``or'' conditions in Equation \eqref{eq:ConditionsB_Varma} implies the following set of conditions:
%             \begin{equation}\label{eq:ConsequenceB_Varma}
%                 \begin{cases}
%                     (PA_{\mathcal{G}^+}(\lambda)\cup SP_{\mathcal{G}^+}(\lambda))\cap A^*=\emptyset,\\
%                     AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(A^*)_{[s_0-l,s_0-1]})=\emptyset\\
%                     \qquad\text{and no bi-directed edges between these ancestral sets,}\\
%                     SP_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(A^*)_{[s_0-l,s_0-1]})=\emptyset,\\
%                     SP_{\mathcal{G}^*}(A^*)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})=\emptyset
%                 \end{cases}.
%             \end{equation}
%             Indeed, each of the ``or'' conditions in Equation \eqref{eq:ConditionsB_Varma} opens a path from $C^*$ to $\lambda$ given $B$ in $\mathcal{G}^*$, as all intermediate nodes are non-colliders not in $B$:
%             \begin{itemize}
%                 \item $PA_{\mathcal{G}^+}(\lambda)\cap C^*\neq\emptyset\Rightarrow C^*\to\lambda$
%                 \item $  SP_{\mathcal{G}^+}(\lambda)\cap C^*\neq\emptyset\Rightarrow C^*\leftrightarrow\lambda$
%                 \item $SP_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\neq\emptyset$ implies: $$C^*\underbrace{\leftrightarrow\bullet}_{\substack{\text{possibly}\\\text{omitted}}}\to\dots\to \lambda,$$
%                 \item $SP_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]})\neq\emptyset$ implies: $$C^*\leftarrow\dots\leftarrow\bullet\leftrightarrow\lambda,$$
%                 \item $AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(C^*)_{[s_0-l,s_0-1]})\neq\emptyset$, or if there is a bi-directed edge between these ancestors, imply: $$C^*\leftarrow\dots\leftarrow\bullet\to\dots\to\lambda\text{ or } C^*\leftarrow\dots\leftarrow\bullet\leftrightarrow\bullet\to\dots\to\lambda.$$
%             \end{itemize}
%             In addition, violation of any of the conditions in Equation \eqref{eq:ConsequenceB_Varma} creates a path in $\mathcal{G}^*$ from $A^*$ to $\lambda$ given $B$, with all intermediate nodes being non-colliders not in $B$. Indeed: 
%             \begin{itemize}
%                 \item $PA_{\mathcal{G}^+}(\lambda)\cap A^*\neq\emptyset\Rightarrow A^*\to\lambda$
%                 \item $  SP_{\mathcal{G}^+}(\lambda)\cap A^*\neq\emptyset\Rightarrow A^*\leftrightarrow\lambda$
%                 \item $SP_{\mathcal{G}^*}(A^*)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\neq\emptyset$ implies: $$A^*\underbrace{\leftrightarrow\bullet}_{\substack{\text{possibly}\\\text{omitted}}}\to\dots\to \lambda,$$
%                 \item $SP_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]}\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(A^*)_{[s_0-l,s_0-1]})\neq\emptyset$ implies: $$A^*\leftarrow\dots\leftarrow\bullet\leftrightarrow\lambda,$$
%                 \item $AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(\lambda)_{[s_0-l,s_0-1]})\cap AN_{\mathcal{G^*}}(PA_{\mathcal{G}^*}(A^*)_{[s_0-l,s_0-1]})\neq\emptyset$, or if there is a bi-directed edge between these ancestors, imply: $$A^*\leftarrow\dots\leftarrow\bullet\to\dots\to\lambda\text{ or } A^*\leftarrow\dots\leftarrow\bullet\leftrightarrow\bullet\to\dots\to\lambda.$$
%             \end{itemize}
%             The $m$-separation hypothesis then means that Equation \eqref{eq:ConditionsB_Varma} implies the conditions in Equation \eqref{eq:ConsequenceB_Varma}, as otherwise we would be able to find a path in $\mathcal{G}^*$ from $A^*$ to $C^*$ such that all intermediate nodes are non-colliders not in $B$, except $\lambda$, which is always a collider and $\lambda\in B$, violating $A^*\perp_{\mathcal{G}^*}C^*|B$.  However, we now note how Equation \eqref{eq:ConsequenceB_Varma} is precisely Equation \eqref{eq:ConditionsA_Varma} replacing $C^*$ for $A^*$. Thus, identical reasoning as in (a) leads again to $A^*\indep C^*|B$. 
%             %which are precisely the conditions in Equation \eqref{eq:ConsequenceA} for $A^*$ instead than for $C^*$. Identical reasoning as in (a) leads to $A^*\indep C^*|B$.
%         \end{itemize}
%     \end{itemize}
%     Therefore, $n+1\in\mathcal{A}$, what means $\mathcal{A}=\mathbb{N}$. This concludes the proof.\qed
% \end{proof}
\begin{remark}
    In the context of $q=0$, i.e. having a VAR($p$) process without instantaneous effects, this proof reduces exactly to that given in \cite{thams2022identifying}, as for example the marginalized ADMG is exactly the full-time DAG.
\end{remark}


